LDPC Codes Achieve List Decoding Capacity

We show that Gallager's ensemble of Low-Density Parity Check (LDPC) codes achieves list-decoding capacity with high probability. These are the first graph-based codes shown to have this property. This result opens up a potential avenue towards truly linear-time list-decodable codes that achieve list-decoding capacity. Our result on list decoding follows from a much more general result: any $\textit{local}$ property satisfied with high probability by a random linear code is also satisfied with high probability by a random LDPC code from Gallager's distribution. Local properties are properties characterized by the exclusion of small sets of codewords, and include list-decodability, list-recoverability and average-radius list-decodability. In order to prove our results on LDPC codes, we establish sharp thresholds for when local properties are satisfied by a random linear code. More precisely, we show that for any local property $\mathcal{P}$, there is some $R^*$ so that random linear codes of rate slightly less than $R^*$ satisfy $\mathcal{P}$ with high probability, while random linear codes of rate slightly more than $R^*$, with high probability, do not. We also give a characterization of the threshold rate $R^*$.

==> prelims.tex <==


For a prime power $q$ we denote by $\F_{q}$ the finite field of $q$ elements.
For any finite alphabet~$\Sigma$, and for any pair of strings $x,y\in\Sigma^{n}$, the \textsf{relative
distance} between $x$ and $y$ is the fraction of coordinates $i \in[n]$ on which $x$ and $y$
differ, and is denoted by $\dist(x,y):= \left|\left\{ i\in\left[n\right]:x_{i}\ne y_{i}\right\} \right|/n$. The 
\textsf{relative weight} of $x$ is $\wt x:=\dist(x,0)$. 
Throughout the paper, we use $\exp n$ to denote $2^{\Theta(n)}$, and whenever we use $\log$, it is base $2$, unless noted otherwise. 


\subsection{Error-correcting codes}

An error-correcting code is simply a subset $C\subseteq\Sigma^{n}$. We call $\Sigma$ the  \textsf{alphabet} of the code, and $n$ its 
\textsf{block length}. The elements of $C$ are called \textsf{codewords}.
If $\Sigma=\F_q$ for a prime power $q$, and $C$ is a linear subspace of $\F_q^n$, we say that $C$ is \textsf{linear}.
The \textsf{rate}
of $C$ is the ratio $R:=\frac{\log|C|}{\log(|\Sigma|^{n})}$, which
for linear codes equals $\frac{\dim(C)}{n}$.
 The
\textsf{relative distance} $\dist(C)$ of $C$ is the minimum $\delta >0$ such that for
any pair of distinct codewords $c_{1},c_{2}\in C$ it holds that
$\dist(c_{1},c_{2})\ge\delta$.   If $C$ is linear, then $\dist(C)$ equals the minimum
 relative weight $\wt{c}$ of a non-zero codeword $c \in C$.


A \textsf{parity-check matrix} for a linear code $C \subseteq \F_q^n$ is an $( (1-R) \cdot n) \times n$ matrix $H$ over $\F_q$ such that $C = \ker(H)$. 
A \textsf{random linear code} $C \subseteq \F_q^n$ of rate $R$ is obtained by sampling a uniform random parity-check matrix $H \in \F_q^{ ((1-R) \cdot n) \times n}$. Note that $C$ has rate at least $R$.

\subsection{Random LDPC}\label{sec:rldpc}

A \textsf{random $s$-LDPC} $C \subseteq \F_q^n$ of rate $R$ is obtained by sampling a parity-check matrix $H \in \F_q^{((1-R) \cdot n) \times n}$ as follows. 
Let $F \in \{0,1\}^{(n/s) \times n}$ be the matrix 
\begin{equation}\label{eq:filter}
F=(F_1 \mid F_2 \mid \ldots \mid F_{n/s}),
\end{equation}
where each $F_i \in \{0,1\}^{(n/s)\times s}$ has all-ones $i$-th row, and the rest of the rows are all-zeros. \TODO{Add drawing of $F$} Let $\Pi \in \{0,1\}^{n \times n}$ be a random permutation matrix, and let $D \in \F_q^{n \times n}$ be a diagonal matrix with diagonal entries that are uniform in $\F_q^*$. 
Then 
\[ H = \left( \begin{array}{ccc}
H_1  \\
H_2  \\
\vdots \\
H_{(1-R)\cdot s}
  \end{array} \right),\]
  where each $H_i$ is sampled independently according to the distribution $F \cdot \Pi \cdot D$. 
 Note that $C$ has rate at least $R$.

\begin{remark} The definition above coincides with Gallager's definition when $q=2$.  However, for larger $q$ our definition is slightly different because we take the diagonal  entries of $D$ to be random in $\F_q^*$, while Gallager chose them to be all $1$. 
\end{remark}

\subsection{Information theory}

For a discrete random variable $X$, we let
$$H(X)= -\sum_{x \in \supp(X)} \Pr[X=x] \cdot \log(\Pr[X=x])$$ denote the \textsf{entropy} of $X$, and we let $H_q(X):=\frac{H(X)} {\log q}$ denote the \textsf{base-$q$ entropy} of $X$.
Similarly, for a pair of discrete random vairables $X,Y$, we let
$I_q(X;Y)= \frac{I(X;Y)} {\log q}$ denote the \textsf{base-$q$ mutual information} of $X$ and $Y$. 

For $x\in [0,1]$, we let
$$
h_q(x)=x\log_q(q-1)-x\log_q(x) -(1-x)\log_q(1-x)
$$
denote the \textsf{$q$-ary entropy function}.

\subsection{Fourier analysis}

In what follows assume that $q = p^h$ for a prime $p$.  The \textsf{trace map} of $\F_q$ over $\F_p$ is the function $\tr:\F_q \to \F_p$  given by
\[ \tr(\alpha) = \alpha + \alpha^p + \alpha^{p^2} + \cdots + \alpha^{p^{h-1}}. \]
 For a function $f: \F_q^n \to \CC$, we define the \textsf{Fourier transform} $\hat{f}: \F_q^n \to \CC$ of $f$ by
\[ \hat{f}(y) = \Eover{x \in \F_q^n} {f(x) \cdot \chi_x(y)},\]
where 
$\chi_x(y) = \omega_p^{\tr(\ip{x}{y})} $, and $\omega_p = e^{2\pi i / p}$. Then we have the decomposition
\[f (x) = \sum_{y\in \F_q^n} \hat f(y) \cdot  \chi_y(x).\]

We define an inner product on the space of $\CC$-valued functions on $\F_q^n$ by 
\[
	\ip{f}{g} = \Eover{x \in \F_q^n}{f(x) \cdot \overline{g(x)}} .
\]	
 \textsf{Plancherel's identity} then asserts that
\[
	\ip{f}{g} = \sum_{x \in \F_q^n}\hat{f}(x) \cdot \overline{\hat{g}(x)}.
\]
An important special case is \textsf{Parseval's identity}:
\[
	\ip ff = \sum_{x \in \F_q^n}|\hat{f}(x)|^2 \ .
\]

The \textsf{convolution}  of a pair of functions $f,g:\F_q^n \to \CC$ is given by
\[
	(f*g)(x) = \Eover{y \in \F_q^n}{f(y) \cdot g(x-y)} \ .
\]
Convolution interacts nicely with the Fourier transform:
\[
	\widehat{f*g}(x) = \hat{f}(x) \cdot \hat{g}(x) \ .
\]
Finally, we define inductively $f^{*1}:=f$, and $f^{*s} = f^{*(s-1)}*f$ for an integer $s\geq 2$. 
